Graph Condensation: A Survey

The rapid growth of graph data poses significant challenges in storage, transmission, and particularly the training of graph neural networks (GNNs). To address these challenges, graph condensation (GC) has emerged as an innovative solution. GC focuses on synthesizing a compact yet highly representative graph, enabling GNNs trained on it to achieve performance comparable to those trained on the original large graph. The notable efficacy of GC and its broad prospects have garnered significant attention and spurred extensive research. This survey paper provides an up-to-date and systematic overview of GC, organizing existing research into five categories aligned with critical GC evaluation criteria: effectiveness, generalization, efficiency, fairness, and robustness. To facilitate an in-depth and comprehensive understanding of GC, this paper examines various methods under each category and thoroughly discusses two essential components within GC: optimization strategies and condensed graph generation. We also empirically compare and analyze representative GC methods with diverse optimization strategies based on the five proposed GC evaluation criteria. Finally, we explore the applications of GC in various fields, outline the related open-source libraries, and highlight the present challenges and novel insights, with the aim of promoting advancements in future research. The related resources can be found at https://github.com/XYGaoG/Graph-Condensation-Papers.

==> 10bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/xinyi.jpg}}]{Xinyi Gao} received his B.S. and M.S. degrees in Information and Communications Engineering from Xi'an Jiaotong University, China. Currently, he is a Ph.D. candidate at the School of Electrical Engineering and Computer Science, the University of Queensland. His research interests include
data mining, graph representation learning, and multimedia signal processing.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/junliang.jpg}}]{Junliang Yu} completed his B.S. and M.S degrees at Chongqing University, and PhD degree at The University of Queensland. Currently, he is a postdoctoral research fellow at the School of Electrical Engineering and Computer Science, the University of Queensland. His research interests include recommender systems, tiny machine learning, and self-supervised learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/rocky.jpg}}]{Tong Chen} received the Ph.D. degree in computer science from The University of Queensland, Brisbane, QLD, Australia, in 2020.
He is currently a Senior Lecturer with the Data Science Research Group, School of Electrical Engineering and Computer Science, The University of Queensland. His research interests include data mining, recommender systems, user behavior modeling, and predictive analytics.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/guanhua.jpg}}]{Guanhua Ye} received the Ph.D. degree in computer science from The University of Queensland, Brisbane, QLD, Australia, in 2023. He is currently an associate professor of the School of Computer Science (National Pilot Software Engineering School), Beijing University of Posts and Telecommunications. His research interests include machine learning, time series analysis, and distributed collaboration.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/wentao.png}}]{Wentao Zhang} is an assistant professor in the Center for Machine Learning Research at Peking University (PKU). Wentao’s research focuses on Graph ML, Data-centric ML, ML systems and AI4Science. Wentao has published 60+ papers in the top DB (SIGMOD, VLDB, ICDE), DM (KDD, WWW), and ML (ICML, NeurIPS, ICLR) venues. Wentao is the contributor or designer of several system projects, including Angel, SGL, and OpenBox. His research works have been powering several billion-scale applications in Tencent, and some of them have been recognized by multiple best paper awards, including the Best Paper Runner Up Award at APWeb-WAIM 2023, and the Best Student Paper Award at WWW 2022.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/hongzhi.jpg}}]{Hongzhi Yin} received a PhD degree in computer science from Peking University, in 2014. He works as an ARC Future Fellow and Full Professor at The University of Queensland, Australia. He has made notable contributions to recommendation systems,  graph learning, and decentralized and edge intelligence. He has published 300+ papers with an H-index of 80 and received the prestigious IEEE Computer Society’s AI’s 10 to Watch Award,  AIPS Young Tall Poppy Science Award,  ARC Future Fellowship 2021 and DECRA Award 2016.
\end{IEEEbiography}
